Manifold learning and optimization using tangent space proxies

We present a framework for efficiently approximating differential-geometric primitives on arbitrary manifolds via construction of an atlas graph representation, which leverages the canonical characterization of a manifold as a finite collection, or atlas, of overlapping coordinate charts. We first show the utility of this framework in a setting where the manifold is expressed in closed form, specifically, a runtime advantage, compared with state-of-the-art approaches, for first-order optimization over the Grassmann manifold. Moreover, using point cloud data for which a complex manifold structure was previously established, i.e., high-contrast image patches, we show that an atlas graph with the correct geometry can be directly learned from the point cloud. Finally, we demonstrate that learning an atlas graph enables downstream key machine learning tasks. In particular, we implement a Riemannian generalization of support vector machines that uses the learned atlas graph to approximate complex differential-geometric primitives, including Riemannian logarithms and vector transports. These settings suggest the potential of this framework for even more complex settings, where ambient dimension and noise levels may be much higher.

==> other_docs/novelty.tex <==

% For SIMODS: Novelty statement 
% Please provide a brief response	
% * What is the novel scientific contribution of this work? 
% (If the work builds considerably on one or more previously published papers, please state how the present work extends the previous ones.)

%Lorenzo's most recent version
% This paper describes a novel numerical data structure, the atlas graph, for representing arbitrary Riemannian manifolds in memory via a finite set of overlapping coordinate charts. In contrast to existing methods, the atlas graph is directly applicable to manifolds lacking closed forms for standard differential-geometric primitives.  he paper demonstrates that the atlas graph captures several manifold invariants, including homology groups, pairwise geodesic distances, and pointwise scalar curvature and allows for quick approximation of the differential-geometric primitives necessary for Riemannian optimization.


%Ryan's most recent version
This paper introduces a new technique for learning and representing Riemannian manifolds that, unlike state-of-the-art dimensionality reduction techniques, preserves geometric and topological invariants and enables faster, more broadly applicable Riemannian optimization. Concretely, we describe a novel numerical data structure, the atlas graph, that encodes a Riemannian manifold in memory using a finite set of overlapping coordinate charts. Our theoretical and empirical work demonstrates that the atlas graph preserves several manifold invariants, such as homology groups, pairwise geodesic distances, and pointwise scalar curvature, which are not maintained by state-of-the-art dimensionality reduction techniques. In contrast to existing frameworks for Riemannian optimization, the atlas graph applies to manifolds lacking closed forms for standard differential-geometric primitives, such as manifolds learned from point cloud data. Moreover, we show that performing Riemannian optimization using primitives computed with atlas graphs can significantly reduce runtime, with trivial loss in accuracy.

